Open Source Software Sustainability: Combining Institutional Analysis and Socio-Technical Networks

Open Source Software (OSS) forms much of the fabric of our digital society, especially successful and sustainable ones. But many OSS projects do not become sustainable, resulting in abandonment and even risks for the world's digital infrastructure. Prior work has looked at the reasons for this mainly from two very different perspectives. In software engineering, the focus has been on understanding success and sustainability from the socio-technical perspective: the OSS programmers' day-to-day activities and the artifacts they create. In institutional analysis, on the other hand, emphasis has been on institutional designs (e.g., policies, rules, and norms) that structure governance. Even though each is necessary for a comprehensive understanding of OSS projects, the connection and interaction between the two approaches have been barely explored. In this paper, we make the first effort toward understanding OSS project sustainability using a dual-view analysis, by combining institutional analysis with socio-technical systems analysis. In particular, we (i) use linguistic approaches to extract institutional rules and norms from OSS contributors' communications to represent the evolution of their governance systems, and (ii) construct socio-technical networks based on longitudinal collaboration records to represent each project's organizational structure. We combined the two methods and applied them to a dataset of developer traces from 253 nascent OSS projects within the Apache Software Foundation (ASF) incubator. We find that the socio-technical and institutional features relate to each other, and provide complementary views into the progress of the ASF's OSS projects. Refining these combined analyses can help provide a more precise understanding of the synchronization between the evolution of institutional governance and organizational structure.

==> RQs.tex <==
%\documentclass[main.tex]{subfiles}
%\begin{document}
Reflecting on the previous discussion, the primary goal of this paper is to demonstrate that the evolution of a project from a nascent state to a sustainable state can be studied effectively by combining the two different methodologies of socio-technical network analysis and institutional analysis.

We reported in prior sections that a variety of scholars have utilized a socio-technical systems approach to analyze collective behavior in OSS projects. 
We also described how institutional analysis is useful in understanding collective action in OSS settings. 
To enable to dual-view on sustainability, we first describe and evaluate our automated approach to identifying institutional statements in project emails.

\textbf{RQ$_{\textcolor{myred}{1}}$: Are there institutional statements contained in ASF Incubator project email discussions? Can we effectively identify them?} 

With the next two research questions, we assess the utility of our convergent approach to the Institutional Analysis (IAD) and STS frameworks. 
In the case of the ASF incubation program, there are two eventual outcomes: either a project graduates from the ASF incubator and becomes a full-fledged ASF associated project, or it “retires” without achieving that goal. 
In this context, we operationalize a sustainable state as one where an OSS project graduates from the ASF incubator program, rather than retires.
We ask:

\textbf{RQ$_{\textcolor{myred}{2}}$: Is OSS project evolution toward sustainability readily observable through the dual lenses of institutional and socio-technical analysis? And how do such temporal patterns differ?}

Per institutional analysis theory, strategies, norms, and rules can affect the social and technical organizations of projects.
Governance and organization, per social theories, must work hand-in-hand to make viable socio-technical systems.  Ill-designed institutional arrangements would introduce inefficiencies into the system, and such inefficiencies may amplify deviant behaviors and irregular structure in the systems. 
Such influential links from institutional design to the organizational structure can be, in fact, bi-directional.
In effect, in a sustainable system, an ill-formed organizational structure may instigate new rules to adjust and improve such structure, further improving efficiencies in the systems.

Thus, we hypothesize that the feedback, if any, between project governance and project organization should be observable, specifically in that intensified governance discussion should precede and/or follow changes to the project organizational structure.
As a reminder, we consider institutional statements as indicators of intensified discussions of OSS project self-governance or new incubator requirements on that self-governance. We also consider socio-technical network parameters as indicators of organizational structure.
Thus, we ask:

\textbf{RQ$_{\textcolor{myred}{3}}$: Are periods of increased Institutional Statements frequency followed by changes in the project organizational structure, and vice-versa?} 

In the following section, we introduce the methodologies approaching the above three research questions. 
%\end{document}
